Ad Lucem: QED Parton Distribution Functions in the MMHT Framework

We present the MMHT2015qed PDF set, resulting from the inclusion of QED corrections to the existing set of MMHT Parton Distribution Functions (PDFs), and which contain the photon PDF of the proton. Adopting an input distribution from the LUXqed formulation, we discuss our methods of including QED effects for the full, coupled DGLAP evolution of all partons with QED at $\mathcal{O}(\alpha)$, $\mathcal{O}(\alpha\alpha_{S})$, $\mathcal{O}(\alpha^2)$. While we find consistency for the photon PDF of the proton with other recent sets, building on this we also present a set of QED corrected neutron PDFs and provide the photon PDF separated into its elastic and inelastic contributions. The effect of QED corrections on the other partons and the fit quality is investigated, and the sources of uncertainty for the photon are outlined. Finally we explore the phenomenological implications of this set, giving the partonic luminosities for both the elastic and inelastic contributions to the photon and the effect of our photon PDF on fits to high mass Drell-Yan production, including the photon--initiated channel.

==> NLO_table.tex <==

\begin{longtable}{ |p{7cm}||p{3.5cm}|p{3.5cm}|  }%\label{tab_fit}
 \hline
 \multicolumn{3}{|c|}{Change in $\chi^2$ due to QED evolution compared to MMHT14+HERA I+II} \\
 \hline
 \textbf{Data set}&\textbf{$\chi^2/N_{pts}$ NLO before fit (QCD)}&\textbf{$\chi^2/N_{pts}$ NLO after fit(QCD+QED)}\\
  \hline	
 BCDMS $\mu p$ $F_2$ \cite{BCDMS_1} &  177 / 163 & 184 / 163 (+7)\\%\hline
 BCDMS $\mu d$ $F_2$ \cite{BCDMS_2} &  139 / 151 & 140 / 151 \\%\hline
 NMC $\mu p$ $F_2$ \cite{NMC_1}&  135 / 123 & 136 / 123 \\%\hline
 NMC $\mu d$ $F_2$ \cite{NMC_1}&  118 / 123 & 121 / 123 (+3) \\%\hline
 NMC $\mu n/\mu p$ $F_2$ \cite{NMC_2}&  128 / 148 & 131 / 148 (+3) \\%\hline
 E665 $\mu p$ $F_2$ \cite{E665}&  60 / 53 & 61 / 53 \\%\hline
 E665 $\mu d$ $F_2$ \cite{E665}&  52 / 53 & 52 / 53 \\%\hline
 SLAC $e p$ $F_2$ \cite{SLAC_1}\cite{SLAC_2}&  31 / 37 & 30 / 37 \\%\hline
 SLAC $e d$ $F_2$ \cite{SLAC_1}\cite{SLAC_2}&  31 / 38 & 30 / 38 \\%\hline
 NMC/BCDMS/SLAC/HERA $F_L$ \cite{NMC_1,BCDMS_1,SLAC_2,HERA_FL_1,HERA_FL_2,HERA_FL_3}& 73 / 57 & 72 / 57 \\\hline
 E866/NuSea $pp$ DY \cite{E866_1}&  218 / 184 & 217 / 184 (-1) \\%\hline
 E866/NuSea $pd/pp$ DY \cite{E866_2} &  12 / 15 & 12 / 15 \\\hline
 NuTeV $\nu N$ $F_2$ \cite{nutev}&  39 / 53 & 36 / 53 (-3)\\%\hline
 CHORUS $\nu N$ $F_2$ \cite{chorus}&  26 / 42 & 25 / 42 \\%\hline
 NuTeV $\nu N$ $xF_3$ \cite{nutev}&  36 / 42 & 36 / 42 \\%\hline
 CHORUS $\nu N$ $xF_3$ \cite{chorus}&  23 / 28 & 23 / 28 \\%\hline
 CCFR $\nu N \rightarrow \mu\mu X$ \cite{CCFR}&  69 / 86 & 69 / 86 \\%\hline
 NuTeV $\nu N \rightarrow \mu\mu X$ \cite{CCFR}&  41 / 84* & 40 / 84* \\\hline
 HERA I+II CC $e^+ p$ \cite{HERA_I_II} & 51 / 39 & 50 / 39  \\%\hline
 HERA I+II CC $e^- p$ \cite{HERA_I_II} & 76 / 42 & 79 / 42 (+3) \\%\hline
 HERA I+II NC $e^+p$ 920 GeV \cite{HERA_I_II} & 546 / 402 & 544 / 402 (-2) \\%\hline
 HERA I+II NC $e^-p$ 920 GeV \cite{HERA_I_II} & 248 / 159  & 248 / 159 \\%\hline
 HERA I+II NC $e^+p$ 820 GeV \cite{HERA_I_II} & 89 / 75 & 89 / 75 \\%\hline
 HERA I+II NC $e^-p$ 575 GeV \cite{HERA_I_II}  & 268 / 259 & 268 / 259 \\%\hline
 HERA I+II NC $e^-p$ 460 GeV \cite{HERA_I_II} & 254 / 209 & 253 / 209 \\%\hline
 HERA $ep$ $F_2^{charm}$ \cite{F2C}&  72 / 52 & 72 / 52 \\%\hline
 H1 99–00 $e^+ p$ incl. jets & 14 / 24  & 14 / 24 \\%\hline
 ZEUS incl. jets & 45 / 60 & 45 / 60 \\%\hline
 D{\O} II $p\bar{p}$ incl. jets \cite{D0_1}&  119 / 110 & 119 / 110 \\%\hline
 CDF II $p\bar{p}$ incl. jets \cite{CDF_1} &  65 / 76 & 69 / 76 \\%\hline
 CDF II $W$ asm. \cite{CDF_2} & 16 / 13 & 16 / 13 \\%\hline
 D{\O} II $W \rightarrow \nu e$ asym. \cite{D0_2} &  33 / 12 & 33 / 12\\%\hline
 D{\O} II $W \rightarrow \nu \mu$ asym. \cite{D0_3}&  16 / 10 & 16 / 10 \\%\hline
 D{\O} II $Z$ rap. \cite{D0_4}&  16 / 28 & 16 / 28 \\%\hline
 CDF $Z$ rap. \cite{CDF_3}&  37 / 28 & 37 / 28 \\\hline\hline
 ATLAS $W^+$, $W^-$, $Z$ \cite{ATLAS-WZ}&  38 / 30 & 39 / 30 \\%\hline
 CMS $W$ asymm $p_T > 35$ GeV \cite{CMS-W}&  7 / 11 & 7 / 11 \\%\hline
 CMS asymm $p_T >$ 25 GeV, 30 GeV \cite{CMS-asym} &  7 / 24 & 7 / 24 \\%\hline
 LHCb $Z\rightarrow e^+ e^-$ \cite{LHCb-1}&  14 / 9 & 14 / 9 \\%\hline
   LHCb $W$ asymm $p_T > 20$ GeV \cite{LHCb-2} &  12 / 10 & 12 / 10 \\%\hline
 CMS $Z\rightarrow e^+ e^-$ \cite{CMS-Z}&  19 / 35 & 19 / 35 \\%\hline
 ATLAS high-mass Drell-Yan \cite{DY-ATLAS}&  21 / 13 & 22 / 13 \\%\hline
 CMS double diff. Drell-Yan \cite{CMS-DY} &  379 / 132 & 385 / 132 (+5)\\%\hline
 Tevatron, ATLAS, CMS $\sigma_{t\bar{t}}$* \cite{tt-1,tt-2,tt-3,tt-4,tt-5,tt-6,tt-7}&  14 / 18 & 14 / 18 \\\hline\hline
 ATLAS jets (2.76 TeV + 7 TeV) &  110 / 116 & 111 / 116 \\\hline
 CMS jets (7 TeV) &  139 / 133 & 141 / 163 (+2)\\\hline\hline
 \textbf{All data} &  \textbf{4139 / 3609} & \textbf{4151/ 3609} (+12)\\\hline
 
\end{longtable}


==> PARTON_QED_HI.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}-10}}%
      \put(1078,1317){\makebox(0,0)[r]{\strut{}-5}}%
      \put(1078,1929){\makebox(0,0)[r]{\strut{}0}}%
      \put(1078,2542){\makebox(0,0)[r]{\strut{}5}}%
      \put(1078,3155){\makebox(0,0)[r]{\strut{}10}}%
      \put(1078,3767){\makebox(0,0)[r]{\strut{}15}}%
      \put(1078,4380){\makebox(0,0)[r]{\strut{}20}}%
      \put(1210,484){\makebox(0,0){\strut{}0}}%
      \put(1776,484){\makebox(0,0){\strut{}0.1}}%
      \put(2342,484){\makebox(0,0){\strut{}0.2}}%
      \put(2908,484){\makebox(0,0){\strut{}0.3}}%
      \put(3474,484){\makebox(0,0){\strut{}0.4}}%
      \put(4040,484){\makebox(0,0){\strut{}0.5}}%
      \put(4606,484){\makebox(0,0){\strut{}0.6}}%
      \put(5172,484){\makebox(0,0){\strut{}0.7}}%
      \put(5738,484){\makebox(0,0){\strut{}0.8}}%
      \put(6304,484){\makebox(0,0){\strut{}0.9}}%
      \put(6870,484){\makebox(0,0){\strut{}1}}%
      \put(440,2542){\rotatebox{90}{\makebox(0,0){\strut{}$\delta f$(\%)}}}%
      \put(4040,154){\makebox(0,0){\strut{}x}}%
      \put(4040,4710){\makebox(0,0){\strut{}QED corrections to $xf(x,Q^2)$, $Q^2 = 10^4$ GeV\textsuperscript{2} (NO FIT)}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5883,1537){\makebox(0,0)[r]{\strut{}U}}%
      \csname LTb\endcsname%
      \put(5883,1317){\makebox(0,0)[r]{\strut{}D}}%
      \csname LTb\endcsname%
      \put(5883,1097){\makebox(0,0)[r]{\strut{}S}}%
      \csname LTb\endcsname%
      \put(5883,877){\makebox(0,0)[r]{\strut{}GLUON}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/PARTON_QED/PARTON_QED_HI}}%
    \gplfronttext
  \end{picture}%
\endgroup

